Generative Language Models for Paragraph-Level Question Generation

Powerful generative models have led to recent progress in question generation (QG). However, it is difficult to measure advances in QG research since there are no standardized resources that allow a uniform comparison among approaches. In this paper, we introduce QG-Bench, a multilingual and multidomain benchmark for QG that unifies existing question answering datasets by converting them to a standard QG setting. It includes general-purpose datasets such as SQuAD for English, datasets from ten domains and two styles, as well as datasets in eight different languages. Using QG-Bench as a reference, we perform an extensive analysis of the capabilities of language models for the task. First, we propose robust QG baselines based on fine-tuning generative language models. Then, we complement automatic evaluation based on standard metrics with an extensive manual evaluation, which in turn sheds light on the difficulty of evaluating QG models. Finally, we analyse both the domain adaptability of these models as well as the effectiveness of multilingual models in languages other than English. QG-Bench is released along with the fine-tuned models presented in the paper https://github.com/asahi417/lm-question-generation, which are also available as a demo https://autoqg.net/.

==> backup.tex <==

\section{Sensitivity to Aggregation}

\begin{table}[h]
\centering
\scalebox{0.7}{
\begin{tabular}{@{}l@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{}}
\toprule
 & \multicolumn{2}{c}{Aggregation} & \multirow{2}{*}{BLEU4} & \multirow{2}{*}{ROUGE-L} & \multirow{2}{*}{METEOR} \\
  &  (Train) &  (Test) &  &  &  \\\midrule
\multirow{8}{*}{\rotatebox{90}{BART\textsubscript{BASE}}}  & -                   & first              & 24.68  & 52.66   & 26.05  \\
                              & -                   & last               & 23.97  & 52.05   & 25.71  \\
                              & -                   & long               & 24.64  & 51.95   & 26.21  \\
                              & -                   & short              & 23.65  & 52.40   & 25.41  \\
                              & first               & first              & 24.72  & 52.49   & 25.95  \\
                              & last                & last               & 23.71  & 51.88   & 25.71  \\
                              & long                & long               & 24.77  & 51.89   & 26.36  \\
                              & short               & short              & 23.69  & 52.06   & 25.58  \\\midrule
\multirow{8}{*}{\rotatebox{90}{BART\textsubscript{LARGE}}} & -                   & first              & 26.17  & 53.85   & 27.07  \\
                              & -                   & last               & 25.48  & 53.24   & 26.75  \\
                              & -                   & long               & 25.46  & 52.77   & 27.10  \\
                              & -                   & short              & 25.28  & 53.76   & 26.48  \\
                              & first               & first              & 25.88  & 53.66   & 27.07  \\
                              & last                & last               & 25.21  & 53.06   & 26.75  \\
                              & long                & long               & 24.91  & 52.41   & 26.89  \\
                              & short               & short              & 25.53  & 53.80   & 26.89  \\\midrule
\multirow{8}{*}{\rotatebox{90}{T5\textsubscript{SMALL}}}   & -                   & first              & 24.40  & 51.43   & 25.84  \\
                              & -                   & last               & 23.82  & 50.95   & 25.50  \\
                              & -                   & long               & 23.40  & 50.45   & 25.86  \\
                              & -                   & short              & 23.81  & 51.58   & 25.30  \\
                              & first               & first              & 23.82  & 51.06   & 25.47  \\
                              & last                & last               & 23.24  & 50.54   & 25.19  \\
                              & long                & long               & 23.18  & 50.10   & 25.51  \\
                              & short               & short              & 23.55  & 51.37   & 25.31  \\\midrule
\multirow{8}{*}{\rotatebox{90}{T5\textsubscript{BASE}}}    & -                   & first              & 26.13  & 53.33   & 26.97  \\
                              & -                   & last               & 25.64  & 52.92   & 26.72  \\
                              & -                   & long               & 25.36  & 52.44   & 27.05  \\
                              & -                   & short              & 25.40  & 53.35   & 26.42  \\
                              & first               & first              & 25.78  & 53.11   & 26.97  \\
                              & last                & last               & 25.34  & 52.73   & 26.72  \\
                              & long                & long               & 25.09  & 51.99   & 26.63  \\
                              & short               & short              & 25.06  & 53.12   & 26.41  \\\midrule
\multirow{8}{*}{\rotatebox{90}{T5\textsubscript{LARGE}}}   & -                   & first              & 27.21  & 54.13   & 27.70  \\
                              & -                   & last               & 26.65  & 53.75   & 27.44  \\
                              & -                   & long               & 26.10  & 53.21   & 27.77  \\
                              & -                   & short              & 26.55  & 54.26   & 27.16  \\
                              & first               & first              & 26.87  & 53.91   & 27.70  \\
                              & last                & last               & 26.59  & 53.66   & 27.57  \\
                              & long                & long               & 25.89  & 52.98   & 27.81  \\
                              & short               & short              & 26.47  & 54.25   & 27.34 \\\bottomrule
\end{tabular}
}
\caption{Automatic metrics from models optimized with different aggregations at calculating BLEU4 to choose the best configuration.}
\label{tab:aggregation}
\end{table}


\begin{table}[t]
\centering
\scalebox{0.75}{
\begin{tabular}{@{}l@{\hspace{5pt}}@{}l@{\hspace{5pt}}@{}l@{\hspace{5pt}}@{}l@{\hspace{5pt}}@{\hspace{3pt}}l@{\hspace{5pt}}@{\hspace{3pt}}l@{\hspace{5pt}}@{\hspace{3pt}}l@{}@{\hspace{5pt}}@{\hspace{3pt}}l@{}}
\toprule
 & Domain & Model & B4 & MTR & R-L & BS & MS \\\midrule
\multirow{12}{*}{\rotatebox{90}{SQuADShifts}} 
                            & \multirow{3}{*}{Amazon}   & BART\textsubscript{BASE}  & 9.51  & 22.59 & 27.54 & 92.67 & 63.14 \\
                            &                           & BART\textsubscript{LARGE} & 9.44  & 22.72 & 27.50 & 92.55 & 62.96 \\
                            &                           & T5\textsubscript{SMALL}   & 8.41  & 22.17 & 27.04 & 91.89 & 62.11 \\
                            &                           & T5\textsubscript{BASE}    & 9.80  & 23.85 & 28.94 & 92.43 & 63.27 \\
                            &                           & T5\textsubscript{LARGE}   & 10.42 & 24.39 & 29.51 & 92.65 & 63.71 \\                              \cline{2-6}
                            & \multirow{3}{*}{Wiki}     & BART\textsubscript{BASE}  & 11.41 & 26.32 & 28.82 & 93.24 & 65.86 \\
                            &                           & BART\textsubscript{LARGE} & 12.08 & 27.65 & 30.30 & 93.45 & 66.60 \\
                            &                           & T5\textsubscript{SMALL}   & 10.90 & 25.95 & 28.18 & 92.63 & 65.04 \\
                            &                           & T5\textsubscript{BASE}    & 11.67 & 27.04 & 29.49 & 93.07 & 65.94 \\
                            &                           & T5\textsubscript{LARGE}   & 12.04 & 27.67 & 30.10 & 93.13 & 66.31 \\
                            \cline{2-6}
                            & \multirow{3}{*}{News}     & BART\textsubscript{BASE}  & 8.76  & 25.18 & 25.37 & 92.77 & 64.87 \\
                            &                           & BART\textsubscript{LARGE} & 9.33  & 25.22 & 25.57 & 93.14 & 65.29 \\
                            &                           & T5\textsubscript{SMALL}   & 7.71  & 23.70 & 23.43 & 92.20 & 63.71 \\
                            &                           & T5\textsubscript{BASE}    & 8.53  & 25.21 & 24.93 & 92.68 & 64.70 \\
                            &                           & T5\textsubscript{LARGE}   & 9.16  & 25.98 & 25.97 & 93.01 & 65.46 \\
                            \cline{2-6}
                            & \multirow{3}{*}{Reddit}   & BART\textsubscript{BASE}  & 8.77  & 22.54 & 26.02 & 92.30 & 62.32 \\
                            &                           & BART\textsubscript{LARGE} & 9.37  & 24.15 & 27.66 & 92.32 & 62.62 \\
                            &                           & T5\textsubscript{SMALL}   & 7.60  & 21.90 & 24.90 & 91.70 & 61.39 \\
                            &                           & T5\textsubscript{BASE}    & 8.75  & 23.57 & 26.84 & 92.26 & 62.52 \\
                            &                           & T5\textsubscript{LARGE}   & 9.16  & 23.97 & 27.24 & 92.43 & 62.74 \\
                            \midrule
\multirow{18}{*}{\rotatebox{90}{SubjQA}}      
                            & \multirow{3}{*}{Book}     & BART\textsubscript{LARGE} & 0.00  & 20.6  & 23.71 & 92.84 & 62.45 \\
                            &                           & T5\textsubscript{SMALL}   & 0     & 18.52 & 19.77 & 92.4  & 61.46 \\
                            &                           & T5\textsubscript{BASE}    & 0     & 21.2  & 22.95 & 93.32 & 63.14 \\
                            &                           & T5\textsubscript{LARGE}   & 0     & 20.83 & 23.68 & 92.89 & 62.51 \\
                            \cline{2-6}
                            & \multirow{3}{*}{Elec.}    & BART\textsubscript{BASE}  & 3.83  & 25.08 & 29.41 & 93.76 & 66.00  \\
                            &                           & BART\textsubscript{LARGE} & 5.18  & 25.17 & 28.87 & 93.51 & 65.68 \\
                            &                           & T5\textsubscript{SMALL}   & 0     & 26.95 & 29.65 & 94.18 & 68.29 \\
                            &                           & T5\textsubscript{BASE}    & 4.55  & 27.39 & 29.99 & 94.26 & 68.33 \\
                            &                           & T5\textsubscript{LARGE}   & 4.57  & 27.56 & 30.55 & 94.27 & 68.8  \\
                            \cline{2-6}
                            & \multirow{3}{*}{Grocery}  & BART\textsubscript{BASE}  & 1.82  & 20.8  & 24.54 & 94.09 & 65.76 \\
                            &                           & BART\textsubscript{LARGE} & 1.93  & 20.42 & 24.28 & 94.1  & 65.79 \\
                            &                           & T5\textsubscript{SMALL}   & 0     & 23.31 & 22.17 & 93.24 & 65.64 \\
                            &                           & T5\textsubscript{BASE}    & 0.83  & 19.87 & 15.63 & 90.56 & 61.47 \\
                            &                           & T5\textsubscript{LARGE}   & 1.13  & 20.64 & 17.4  & 91.39 & 63.41 \\
                            \cline{2-6}
                            & \multirow{3}{*}{Movie}    & BART\textsubscript{BASE}  & 3.89  & 20.55 & 25.43 & 93.61 & 62.91 \\
                            &                           & BART\textsubscript{LARGE} & 4.21  & 21.64 & 25.92 & 93.23 & 62.4  \\
                            &                           & T5\textsubscript{SMALL}   & 0     & 22.54 & 25.76 & 94.08 & 64.63 \\
                            &                           & T5\textsubscript{BASE}    & 2.65  & 23.11 & 26.33 & 94.13 & 64.91 \\
                            &                           & T5\textsubscript{LARGE}   & 0     & 21.7  & 25.06 & 93.64 & 63.88 \\
                            \cline{2-6}
                            & \multirow{3}{*}{Rest.}    & BART\textsubscript{BASE}  & 3.43  & 21.35 & 24.26 & 93.23 & 62.67 \\
                            &                           & BART\textsubscript{LARGE} & 5.54  & 22.46 & 24.77 & 93.23 & 63.57 \\
                            &                           & T5\textsubscript{SMALL}   & 0     & 13.21 & 11.72 & 87.81 & 55.42 \\
                            &                           & T5\textsubscript{BASE}    & 0     & 14.75 & 11.96 & 88.48 & 56.19 \\
                            &                           & T5\textsubscript{LARGE}   & 4.19  & 21.99 & 24.94 & 93.22 & 63.25 \\
                            \cline{2-6}
                            & \multirow{3}{*}{Trip}     & BART\textsubscript{BASE}  & 4.79  & 25.26 & 26.37 & 93.92 & 64.91 \\
                            &                           & BART\textsubscript{LARGE} & 5.66  & 24.32 & 26.5  & 93.85 & 64.02 \\
                            &                           & T5\textsubscript{SMALL}   & 2.49  & 25.56 & 23.91 & 93.75 & 66.57 \\
                            &                           & T5\textsubscript{BASE}    & 1.74  & 20.13 & 16.06 & 90.76 & 59.7  \\
                            &                           & T5\textsubscript{LARGE}   & 5.35  & 27.45 & 27.69 & 94.46 & 67.76  \\
                            \bottomrule
\end{tabular}
}
\caption{Result of zeroshot-transfer to SubjQA/SQuADShifts dataset.}
\label{tab:domain-transfer}
\end{table}


\begin{table}[t]
\centering
\scalebox{0.7}{
\begin{tabular}{@{}l@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{}}
\toprule
             & Data size            & \multicolumn{3}{c}{Average character length}  \\
             &       (train/valid/test)      & Paragraph & Question & Answer \\
             \midrule
SQuAD        & 75,722/10,570/11,877 & 757                  & 59                   & 20                   \\\midrule
\multicolumn{3}{@{}l}{SubjQA}            &                              &                            \\
- \textit{Book}    & 637/92/191    & 1,514                 & 28                   & 83                   \\
- \textit{Elec.}    & 697/99/238    & 1,282                 & 26                   & 66                   \\
- \textit{Grocery}  & 687/101/379   & 896                  & 25                   & 49                   \\
- \textit{Movie}    & 724/101/154   & 1,746                 & 27                   & 72                   \\
- \textit{Rest.}    & 823/129/136   & 1,006                 & 26                   & 51                   \\
- \textit{Trip}     & 875/143/397   & 1,002                 & 27                   & 51                   \\
\midrule
\multicolumn{3}{@{}l}{SQuADShifts}             &                              &                            \\
- \textit{Amazon}   & 3,295/1,648/4,942 & 775                  & 48                   & 20                   \\
- \textit{Wiki}     & 2,646/1,323/3,969 & 780                  & 54                   & 23                   \\
- \textit{News}     & 3,355/1,678/5,032 & 778                  & 48                   & 19                   \\
- \textit{Reddit}   & 3,268/1,634/4,901 & 773                  & 44                   & 18                   \\
\midrule
\multicolumn{3}{@{}l}{MLQG}          &                              &                            \\
- \textit{Ja}   & 27,809/3,939/3,939   & 424                  & 32                   & 6                    \\
- \textit{Es}   & 77,025/10,570/10,570 & 781                  & 64                   & 21                   \\
- \textit{De}   & 9,314/2,204/2,204    & 1,577                 & 59                   & 66                   \\
- \textit{Ru}   & 40,291/5,036/5,036   & 754                  & 64                   & 26                   \\
- \textit{Ko}   & 54,556/5,766/5,766   & 521                  & 34                   & 6                    \\
- \textit{It}   & 46,550/7,609/7,609   & 807                  & 66                   & 16                   \\
- \textit{Fr}   & 17,543/3,188/3,188   & 797                  & 57                   & 23               \\
\bottomrule
\end{tabular}
}
\caption{Statistics of of all datasets integrating into our question generation benchmark after unification. }
\label{tab:data}
\end{table}
% \begin{table}[t]
% \centering
% \scalebox{0.7}{
% \begin{tabular}{@{}l@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{\hspace{3pt}}c@{}}
% \toprule
%              & \multirow{2}{*}{Data Size}            & \multicolumn{3}{c}{Average Character Length}  \\
%              &            & Paragraph & Question & Answer \\
%              \midrule
% SQuAD        & 75,722/10,570/11,877 & 763/779/699                   & 59/60/61                     & 21/19/17                   \\\midrule
% \multicolumn{3}{@{}l}{SubjQA}                       &                              &                            \\
% - \textit{Books}        & 637/92/191           & 1532/1421/1498                & 28/26/30                     & 89/84/61                   \\
% - \textit{Elec.}  & 697/99/238           & 1295/1318/1231                & 26/26/26                     & 63/35/86                   \\
% - \textit{Grocery}      & 687/101/379          & 904/869/887                   & 26/25/25                     & 49/44/52                   \\
% - \textit{Movie}       & 724/101/154          & 1777/1681/1638                & 27/25/29                     & 73/89/55                   \\
% - \textit{Rest.}  & 823/129/136          & 1011/1003/982                 & 26/27/26                     & 52/50/48                   \\
% - \textit{Trip}  & 875/143/397          & 991/1004/1027                 & 28/27/27                     & 54/44/46                   \\\midrule
% % - \textit{All}          & 4,443/665/1,495      & 1235/1191/1143                & 27/26/27                     & 62/56/57                   \\
% \multicolumn{3}{@{}l}{SQuADShifts}             &                              &                            \\
% - \textit{Wiki}         & 2,646/1,323/5,032    & 776/776/784                   & 58/58/51                     & 26/26/20                   \\
% - \textit{News}         & 3,355/1,678/4,901    & 778/778/777                   & 51/51/45                     & 19/19/19                   \\
% - \textit{Reddit}       & 3,268/1,634/4,942    & 770/770/776                   & 45/45/43                     & 19/19/18                   \\
% - \textit{Amazon}       & 3,295/1,648/18,844   & 770/770/777                   & 43/43/49                     & 18/18/20                   \\\midrule
% % - \textit{All}          & 9,209/6,283/52,200   & 774/774/3562                  & 49/49/37                     & 20/20/34                   \\
% \multicolumn{3}{@{}l}{MLQG}          &                              &                            \\
% - \textit{Ja}     & 27,809/3,939/3,939   & 430/372/430                   & 32/31/32                     & 6/6/6                      \\
% - \textit{Es}      & 77,025/10,570/10,570 & 778/795/784                   & 63/64/64                     & 21/21/21                   \\
% - \textit{De}       & 9,314/2,204/2,204    & 1,379/1,385/2,605             & 59/59/57                     & 67/70/60                   \\
% - \textit{Ru}      & 40,291/5,036/5,036   & 754/755/750                   & 64/64/65                     & 26/26/26                   \\
% - \textit{Ko}       & 54,556/5,766/5,766   & 520/541/515                   & 34/34/34                     & 6/6/6                      \\
% - \textit{It}      & 46,550/7,609/7,609   & 801/797/852                   & 66/65/67                     & 16/16/17                   \\
% - \textit{Fr}       & 17,543/3,188/3,188   & 780/913/775                   & 57/54/57                     & 22/26/22                   \\
% \bottomrule
% \end{tabular}
% }
% \caption{Statistics of train/validation/test split for all the QG datasets we use in our paper.}
% \label{tab:data}
% \end{table}

\begin{table}[t]
\centering
\scalebox{0.75}{
\begin{tabular}{@{}l@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{\hspace{5pt}}r@{}}
\toprule
% Model  & answerability & grammaticality & understandability & B4 & R-L & MTR & BS & MS\\\midrule
Model  & Ans. & Gra. & Und. & B4 & R-L & MTR & BS & MS\\\midrule
T5\textsubscript{LARGE}  & 2.80  & 2.93  & 2.95  & 17.56 & 30.42  & 52.00    & 90.94 & 66.09\\
 - sent-level  & 2.47  & 2.91  & 2.95  & 14.88 & 27.49  & 48.97    & 90.76 & 64.53 \\
 - answer-free                    & 2.46  & 2.91  & 2.95  & 13.62 & 26.82  & 47.37    & 90.20 & 64.00 \\
T5\textsubscript{SMALL}                         & 2.51  & 2.83  & 2.90  & 13.43 & 27.38  & 48.86   
&90.41&64.27\\
BART\textsubscript{LARGE}                       & 2.70  & 2.89  & 2.93  & 16.15 & 29.93  & 51.35    & 90.95 & 65.44 \\
NQG        & 1.21  & 2.35  & 2.63  & 3.33  & 14.30  & 33.53    & 88.27 & 58.25 \\\bottomrule
\end{tabular}
}
\caption{Manual evaluation results along with the automatic metrics. Each score is averaged within the 500 questions for the evaluation.}
\label{tab:manual_evaluation}
\end{table}


% \subsection{Model comparison}

% %\subsubsection{Automatic and QA-based Evaluation}
% %\label{sec:main_result}

% In \autoref{tab:main-squad}, we can confirm that T5\textsubscript{LARGE} establishes new SotA across all the metrics.
% Our main models are also parameter-efficient, since T5\textsubscript{BASE} outperforms ERNIE-GEN \cite{ERNIE-GEN} with less parameters, and T5\textsubscript{SMALL} performs competitively with UniLMv2 \cite{UNILMv2} with nearly half the parameters. 
% UniLMv2, in particular, has been proposed as a highly-effective model in spite of its light weight, so it can be said that T5\textsubscript{SMALL} is also capable of learning the QG task very efficiently. BART models perform very well against the SotA models too, as BART\textsubscript{LARGE} outperforms all the existing SotA models and BART\textsubscript{BASE} is better than most of the SotA models with less parameters except for ERNIE-GEN and UniLMv2. 
% Comparing BART and T5 models, BART\textsubscript{BASE} is slightly better than T5\textsubscript{BASE} and BART\textsubscript{LARGE} is equal to T5\textsubscript{LARGE} in BERTScore, but the other metrics are correlated with the model size, which means there is no significant difference among their performances.

% The results of our unsupervised QA-based evaluation in \autoref{tab:qae} indicate that the QA model accuracy correlates with the size of QG model that generated the synthetic data, as in T5\textsubscript{LARGE} realizes the best QA model in both of F1 and the exact match,
% which is as good as the supervised non-language model based QA models \cite{wang2016machine,yang2017words}. Also, the small models such as T5\textsubscript{SMALL} and BART\textsubscript{BASE} produce QA models with a small decrease in performance, which exhibits the efficiency of our models, similarly to our results with automatic metrics.

% % Why have T5 and BART based QG models been underrated in the SQuAD QG task? \autoref{tab:default} shows the decrease in each metric if the model is fine-tuned without parameter optimization\footnote{We follow the hyperparameter used to fine-tune ERNIE-GEN on SQuAD QG in the original paper.}.
% % We observe decent drops in performance. T5\textsubscript{SMALL} and BART\textsubscript{LARGE} lose around 2 points in BLEU4 and ROUGE\textsubscript{L}. 
% % According to these results, we infer that T5 and BART were worse than more recent language models (ProphetNet, UniLM, or ERNIE-GEN) in QG just because they were under-fitted to the task due to  sub-optimal fine-tuning parameters, rather than they being inferior to those recent language models in terms of learning the QG task. 



% \subsection{Feature analysis}

% \jose{(Not sure if feature is the correct name for this, but basically an analysis on whether models are trained on the whole pargraph, with/without answer, etc.). Analysis on the main Squad dataset}
% %Answer-aware/free Model Comparison


% The sentence is always part of the paragraph, so the paragraph-level model has access to more context than the sentence-level model. 
% \autoref{fig:task_overview} shows an example of each type of input, and 
% \autoref{fig:model_type} gives a high-level view of each model type's definition.
% such model is defined as $f_c :\: c \mapsto \hat{q}$. 
% but generally existing QG models can be grouped into two categories with respect to their input types. 
% the sentence where the question should be anchored is highlighted instead
% the answer is always highlighted in the paragraph as explained in , which we call \textbf{Answer-aware QG models}, while \textbf{Answer-free QG models} do not assume to have the answer \cite{lopez2020transformer,pyatkin-etal-2021-asking}.
% The context is usually either a paragraph \cite{lopez2020transformer} or a sentence \cite{du-etal-2017-learning,lopez2020transformepyatkin-etal-2021-asking}.
% On the other hand, \textbf{Answer-aware QG models} use the answer $a$ in addition to the context $c$ so that the model can generate questions associated with a particular answer \cite{du-cardie-2018-harvesting,chan-fan-2019-recurrent,zhang-bansal-2019-addressing}, and such model is defined as $f_{c,a} :\: (c, a) \mapsto \hat{q}$. 

% Finally, an end-to-end QA generation model is a type of model that learns to generate the question and the answer pair jointly $f_{e2e} :\: c \mapsto (\hat{q}, \hat{a})$ \cite{shakeri-etal-2021-towards}. However, in practice, these models mostly rely on a two-stage pipeline \cite{puri-etal-2020-training,lee-etal-2020-generating,bartolo-etal-2021-improving,lewis-etal-2021-paq,paranjape2021retrieval} that incorporates an answer-aware QG model $f_{c,a}$ and a separately-optimized answer extraction model $g:\: c \mapsto \hat{a}$, i.e. $f_{e2e}(c) := (f_{c,a}(c, g(c)), g(c))$, so we consider this type of model to be part of the family of answer-aware QG models.

